Structure formation in a colliding flow: The Herschel view of the Draco nebula

The Draco nebula is a high Galactic latitude interstellar cloud likely to have been formed by the collision of a Galactic halo cloud entering the disk of the Milky Way. Such conditions are ideal to study the formation of cold and dense gas in colliding flows of warm gas. We present Herschel-SPIRE observations that reveal the fragmented structure of the interface between the infalling cloud and the Galactic layer. This front is characterized by a Rayleigh-Taylor instability structure. From the determination of the typical length of the periodic structure (2.2 pc) we estimated the gas kinematic viscosity and the turbulence dissipation scale (0.1 pc) that is compatible with that expected if ambipolar diffusion is the main mechanism of energy dissipation in the WNM. The small-scale structures of the nebula are typical of that seen in some molecular clouds. The gas density has a log-normal distribution with an average value of $10^3$ cm$^{-3}$. The size of the structures is 0.1-0.2 pc but this estimate is limited by the resolution of the observations. The mass ranges from 0.2 to 20 M$_{\odot}$ and the distribution of the more massive clumps follows a power law $dN/d\log(M) \sim M^{-1.4}$. We identify a mass-size relation with the same exponent as that found in GMCs ($M\sim L^{2.3}$) but only 15% of the mass of the cloud is in gravitationally bound structures. We conclude that the increase of pressure in the collision is strong enough to trigger the WNM-CNM transition caused by the interplay between turbulence and thermal instability as self-gravity is not dominating the dynamics.

==> Physics.tex <==
% ***********************************************************
% ******************* PHYSICS HEADER ************************
% ***********************************************************
\usepackage{amsmath}
%\usepackage{amsthm}
\usepackage{amssymb}
\usepackage[a]{esvect}
\usepackage{tikz}


% Units
\newcommand{\degree}[0]{$^{\circ}$}
\newcommand{\angstrom}[0]{\AA\;}


% Fractions with brackets
\newcommand{\cbra}[1]{\left( #1 \right)}      % put the argument between parentheses (curve brackets)
\newcommand{\sbra}[1]{\left[ #1 \right]}      % put the argument between square brackets
\newcommand{\abra}[1]{\langle #1 \rangle}     % put the argument between angle brackets
\newcommand{\acbra}[1]{\left\{ #1 \right\}}   % put the argument between curly brackets


% Vectors
\let\vaccent=\v % rename builtin command \v{} to \vaccent{}
\renewcommand{\v}[1]{\ensuremath{\vv{#1}}}                 % vectors with arrow
\newcommand{\gvec}[1]{\ensuremath{\mbox{\boldmath$ #1 $}}} % vectors without arrow
\newcommand{\uvec}[1]{\ensuremath{\mathbf{\hat{#1}}}}      % unit vector


% Statistics
\newcommand{\abs}[1]{\left| #1 \right|}         % absolute value
\newcommand{\avg}[1]{\left< #1 \right>}         % average
\newcommand{\mean}[1]{\overline{#1}}            % mean
\newcommand{\rms}[1]{\left< #1^2 \right>^{1/2}} % root mean square


% Derivative
\let\underdot=\d % rename builtin command \d{} to \underdot{}
\renewcommand{\d}[2]{\frac{d #1}{d #2}}    % derivatives
\newcommand{\dd}[2]{\frac{d^2 #1}{d #2^2}} % double derivatives

\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}      % partial derivatives
\newcommand{\pdd}[2]{\frac{\partial^2 #1}{\partial #2^2}} % double partial derivatives

\newcommand{\pdc}[3]{\left( \frac{\partial #1}{\partial #2}\right)_{#3}} % thermodynamic derivatives


% Bras-kets
\newcommand{\ket}[1]{\left| #1 \right>} % Dirac bras
\newcommand{\bra}[1]{\left< #1 \right|} % Dirac kets
\newcommand{\braket}[2]{\left< #1 \right| \left. #2 \right>} % Dirac brackets
\newcommand{\matrixel}[3]{\left< #1 \right|  #2 \left| #3 \right>} % Dirac matrix elements

% Nabla
\newcommand{\grad}[1]{\gv{\nabla} #1} % gradient

\let\divsymb=\div % rename builtin command \div to \divsymb
\renewcommand{\div}[1]{\v{\nabla} \cdot #1} % divergence
\newcommand{\curl}[1]{\v{\nabla} \times #1} % curl


\let\baraccent=\=
\renewcommand{\=}[1]{\stackrel{#1}{=}} % for putting numbers above =
\let\arrowaccent=\>
\renewcommand{\>}[1]{\stackrel{#1}{\Rightarrow}} % for putting numbers above =>

% Roman numbers
\makeatletter
\newcommand{\rmnum}[1]{{\footnotesize{\expandafter\@slowromancap\romannumeral #1@}}}
\newcommand{\Rmnum}[1]{{\expandafter\@slowromancap\romannumeral #1@}}
\makeatother

% Roman numbers
\newcommand{\circled}[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=2pt](char){#1};}}

% ***********************************************************
% ********************** END HEADER *************************
% ***********************************************************

